Timed Orchestration for Component-based Systems

Individual machines in flexible production lines explicitly expose capabilities at their interfaces by means of parametric skills. Given such a set of configurable machines, a line integrator is faced with the problem of finding and tuning parameters for each machine such that the overall production line implements given safety and temporal requirements in an optimized and robust fashion. We formalize this problem of configuring and orchestrating flexible production lines as a parameter synthesis problem for systems of parametric timed automata, where interactions are based on skills. Parameter synthesis problems for interaction-level LTL properties are translated to parameter synthesis problems for state-based safety properties. For safety properties, synthesis problems are solved by checking satisfiability of $\exists\forall$SMT constraints. For constraint generation, we provide a set of computationally cheap over-approximations of the set of reachable states, together with fence constructions as sufficient conditions for safety formulas. We demonstrate the feasibility of our approach by solving typical machine configuration problems as encountered in industrial automation.

==> algo_monitor_old.tex <==
\subsection{Translating $\phi_{int}$ into a deterministic monitor component and a deadlock detection property}\label{sub.sec.monitor}

Intuitively, the idea behind a deterministic monitor for an LTL
property $\phi$ is to create a deterministic automaton which keeps
track of the final states visited in the B\"uchi automaton
$\mathcal{A}_{\neg \phi}$ corresponding to $\neg\phi$ during system
execution. The deterministic automaton has a risk state representing
that a final state in $\mathcal{A}_{\neg \phi}$ has been visited for
$k$ times. When the risk state is never reached for all possible runs,
all final states in $\mathcal{A}_{\neg \phi}$ are visited finitely
often (i.e., less than $k$ times). This observation is sufficient to
conclude that the system satisfies $\phi$.

%one should only visit every final state finitely often. \obs{as it is, not clear if finiteness is a requirement or a general statement; i'd rather make it more explicit like this: Our construction is such that final states are visited finitely often.}

%% More precisely, given $\mathcal{S}$ and an interaction-level property
%% $\phi_{int}$, denote $\Sigma_{\phi_{int}} \subseteq \Sigma$ to be the
%% set of interactions used in $\phi_{int}$. Let~$\#$ be a symbol not
%% within $\Sigma$ and let $k$ be an integer bound denoting the maximum
%% number of allowed visits. The construction of a \emph{deterministic
%%   monitor component} $C_{\neg\phi_{int},k}$ from $\phi_{int}$ consists
%% of three steps which we explain and illustrate by means of the example
%% in Figure~\ref{fig:TimedPhilosopher} below.

More precisely, given $\mathcal{S}$, an interaction-level property
$\phi_{int}$, and an integer $k$, the construction of a
\emph{deterministic monitor component} $C_{\neg\phi_{int},k}$ from
$\phi_{int}$ consists of three steps which we explain and illustrate
by means of the example in Figure~\ref{fig:TimedPhilosopher} below.
Before, we introduce some notation for the ease of reference. We use
$\Sigma_{\phi_{int}} \subseteq \Sigma$ to be the set of interactions
used in $\phi_{int}$ and $\#$ as a symbol not within $\Sigma$. We
recall that we use $\sigma$ to denote interactions. To avoid ambiguity, we call a state in the monitor component ``location'' and use the name ``state'' for B\"uchi automaton.
	
\begin{itemize}
	\item \textbf{(Step 1)} Construct a B\"uchi automaton $\mathcal{A}_{\neg\phi_{int}}$ for the negated property of  $\phi_{int}$. Post-process the automaton by replacing every label $\neg \sigma$ with $\Sigma_{\phi_{int}}\setminus \{\sigma\} \cup \{\#\}$. For the timed dining philosopher's problem, Figure~\ref{fig:negated.property}-(a) shows the result $\mathcal{A}_{\neg \phi_{prompt}}$ for property $\phi_{prompt}$, while (b) shows the result after post processing. 
	%\obs{confused: if $\mathcal{A}_{\neg \phi_{prompt}}$ is the buchi for $\neg \phi$, then it doesn't contain $\#$. Maybe rephrase like: construct a buchi automaton for the negated... Post-proc ... Let the resulting automaton be $\mathcal{A}_{\neg \phi_{prompt}}$. -- and change caption to Fig.2a to $\mathcal{A}_{\neg \phi_{prompt}}$.} %Figure~\ref{fig:negated.property}-(b,c) explains the replacement for 
	% The thing is that, even 
	
		\begin{figure}[t]
			
			\centering
			\includegraphics[width=0.95\columnwidth]{fig/NegatedProperty}
			
			\caption{(a)(b) B\"uchi automaton for $\neg \phi_{prompt}$ before and after postprocessing. (c) Monitor component $\mathcal{C}_{\neg \phi_{prompt}, 1}$.  }
			\label{fig:negated.property}
			
		\end{figure}
	
	\item \textbf{(Step 2)} Starting from the initial state of $\mathcal{A}_{\neg\phi_{int}}$, use $\Sigma_{\phi_{int}}\cup \{\#\}$ to \emph{unroll} all traces of $\mathcal{A}_{\neg\phi_{int}}$ and create a deterministic monitor $C_{\neg \phi_{int},k}$. As this step is analogous to the approach  in bounded LTL synthesis~\cite{ScheweF07a} which unrolls a B\"uchi automaton for the negated property, here we only outline the algorithm accompanied by examples. Figure~\ref{fig:negated.property}-(c) shows the result of unrolling for $k=1$.
	\begin{enumerate}
		
		\item Each location in $C_{\neg \phi_{int},k}$ records the set of states being visited in the B\"uchi automaton. It also counts for each state, the number of times a final state in $\mathcal{A}_{\neg\phi_{int}}$ has been visited previously. In Figure~\ref{fig:negated.property}-(c), the initial location stores \{$s_0$[$s_3$(0)]\}, where [$s_3$(0)] is to indicate  that at $s_0$, one has not yet reached  $s_3$ previously. The initial location is placed in a queue to be processed. 
		
		\item The algorithm takes an unprocessed location in the queue, and selects every interaction $\sigma \in \Sigma_{\phi_{int}} \cup \{\#\}$ to create a successor location respectively. A state $s'$ is stored in the successor location, if state $s$ is in the unprocessed location and in the post-processed B\"uchi automaton, a transition from $s$ to $s'$ via edge labeled $\sigma$ exists. Also update the number of visited final states.
		In Figure~\ref{fig:negated.property}-(c), when the initial location  \{$s_0$[$s_3(0)$]\} takes interaction \sig{take1}, it goes to  \{$s_0$[$s_3(0)$], $s_1$[$s_3(0)$]\}, as in Figure~\ref{fig:negated.property}-(b), state $s_0$ can move to $s_0$ or $s_1$. 
		It is possible that a destination location has been created previously. E.g., in Figure~\ref{fig:negated.property}-(c), for the initial location  \{$s_0$[$s_3(0)$]\} to take interaction \#, it goes back to \{$s_0$[$s_3(0)$]\}.
		
		\item Whenever a final state in $\mathcal{A}_{\neg\phi_{int}}$ has been visited $k$ times, the unroll process replaces the location of $C_{\neg \phi_{int},k}$ by \sig{risk}, a dedicated location with no outgoing edges. E.g., in Figure~\ref{fig:negated.property}-(c) for \{$s_0$[$s_3(0)$], $s_1$[$s_3(0)$]\} to take interaction \sig{take2}, it moves to a new location 
		\{$s_0$[$s_3(0)$], $s_3$[$s_3(1)$], $s_2$[$s_3(0)$]\}. This new location is then replaced by \sig{risk}, as in this example, we have $k=1$.
		 
	\end{enumerate}
%\obs{\begin{itemize}\item the notation $N$ is misleading also, as it makes one think of a natural number (why not use $f$, \textit{fin}); what does $T$ stand for? why not simply use $l$ (to stand for location) instead? \item i find the notation $init[0]$ misleading (makes me think of arrays), maybe use \textit{occ}? also, i find it confusing to associate non-final locs with the numbers counting occ of final states: what if we have more final states? why not use \textit{occ}$_f$ = val in each state s of $\mon{k}$ to denote that at s, final state f is visited val times. If \textit{occ} is too long, why not use $\#f=val$ instead and use $*$ in place of $\#$ as a label? \end{itemize}}




	\item \textbf{(Step 3)} Create an augmented system $\mathcal{S}_{inv,k} = (V, C\cup \{C_{\neg\phi_{int},k}\}, \Sigma, \Delta_{inv,k})$ from  $\mathcal{S}$, where $\Delta_{inv,k}$ is defined by extending $\Delta$: If $\sigma \in \Sigma_{\phi_{int}}$,  then $\Delta_{inv,k}(\sigma):= \Delta(\sigma)\cup\{C_{\neg\phi_{int},k}.\sigma\}$. Otherwise, set $\Delta_{inv,k}(\sigma):= \Delta(\sigma)\cup\{C_{\neg\phi_{int},k}.\#\}$. That is, all property-unrelated interactions are attached by $\#$.
	\begin{itemize}
		\item For our example, $\Delta_{inv,k}(\sig{take1})$ is set to $\{\phio_1.\port{take1}, Fork_1.\port{take}, C_{\neg\phi_{prompt}}.\port{take1}\}$, while
		  $\Delta_{inv,k}(\sig{eat2})$ is set to $\{\phio_2.\port{eat}, Fork_1.\port{take}, C_{\neg \phi_{prompt}}.\#\}$.
	\end{itemize}

	\item \textbf{(Step 4)} Create state predicate $\phi_{deadlock} :=\bigwedge_{\sigma \in \Sigma} \neg \tEn{\sigma}$ as the deadlock condition.

\end{itemize}


\vspace{2mm}
	
%\noindent The following result relates the timed orchestration synthesis for interaction-level properties to the timed orchestration synthesis for state-based properties.



The following result reduces the timed orchestration synthesis for interaction-level properties to that for state-based properties.


\begin{lemma}
  Given $\vec{v}$ an assignment of $V$, $\mathcal{S}(\vec{v})$ satisfies $\phi_{int}$ if all time runs of $\mathcal{S}_{inv,k}(\vec{v})$ reach neither the location \sig{risk} in $C_{\neg\phi_{int},k}$ nor a state where $\phi_{deadlock}(\vec{v})$ holds. 
  %\obs{i find it too vague ``state defined by $\phi_{dead}$''.}

%\footnote{Observe that, by our construction, once the monitor enters the \textsf{risk} location, the system is deadlocked. Therefore, it actually suffices to only avoid deadlock.\obs{don't understand ``therefore'' nor ``suffices'': suffices for \textit{what}? doesn't ``therefore'' dismiss the need for $\phi_{deadlock}$?}}
\end{lemma}


\proof (Sketch) Assume location \sig{risk} and for all states where $\phi_{deadlock}(\vec{v})$ holds are
not visited by any time run $\rho$ in $\mathcal{S}_{inv,k}(\vec{v})$. 


\begin{enumerate}
	
\item 	Because $\dead$ does not hold and because time runs are maximal, any such time run $\rho$ is infinite. 
%	\item Because $\phi_{deadlock}(\vec{v})$ is never reached, $\bigvee_{\sigma \in \Sigma} \tEn{\sigma}(\vec{v})$ is an  invariant, thus it holds in any reachable state $s$. This  implies that at least one $\tEn{\sigma}(\vec{v})$ is \sig{true}, meaning that the discrete jump defined by  $\sigma$ can be taken from $s$ after some finite delay imposed by the time constraints in $\tEn{\sigma}(\vec{v})$. Consequently, $\rho_{\Sigma}$ is a run in $\mathcal{S}(\vec{v})$.

\item From an infinite time run $\rho$, we show that $\rho$ defines an $\omega$-word $\rho_{\Sigma}$: As $\phi_{deadlock}(\vec{v})$ is never reached,
$\bigvee_{\sigma \in \Sigma} \tEn{\sigma}(\vec{v})$ is an invariant
for all reachable states. Recall our definition where $\tEn{\sigma}$ is the necessary
condition for enabling a location combination to trigger $\sigma$ by
only allowing \emph{finite-time} evolving. Therefore, for all reachable states, one of the interaction (discrete jump) must appear after finite time. Thus,   $\rho$ contains infinitely many discrete jumps. Therefore, $\rho$ defines an $\omega$-word $\rho_{\Sigma}$.

\item Recall that in our monitor construction, every location has edges 
labeled in $\sigma \in \Sigma_{\phi_{int}} \cup \{\#\}$  (Step~2), and \# is actually  paired each property-unrelated interaction in $\Sigma\setminus \Sigma_{\phi_{int}}$ (Step 3). Therefore, if \sig{risk} is not reached, when composing the monitor component with $\mathcal{S}(\vec{v})$ to form the new system $\mathcal{S}_{inv,k}(\vec{v})$, $\mathcal{S}_{inv,k}(\vec{v})$ does not restrict the behavior of $\mathcal{S}(\vec{v})$. That is,  every time run $\rho'$ in $\mathcal{S}(\vec{v})$ can be extended to a time run $\rho$ in  $\mathcal{S}_{inv,k}(\vec{v})$ (and vice versa), while $\rho$ and $\rho'$ define the same $\omega$-word $\rho_{\Sigma}$. 

\item $C_{\neg\phi_{int},k}$ is an unroll of
$\mathcal{A}_{\neg\phi_{int}}$, then as (1) $\rho_{\Sigma}$
exists  and (2) running $\rho_{\Sigma}$ in
$\mathcal{A}_{\neg\phi_{int}}$ does not touch any final
state infinitely many times, $\rho_{\Sigma}$ does not
satisfy $\neg\phi_{int}$. Therefore, for every time run
$\rho'$ in $\mathcal{S}(\vec{v})$, the corresponding $\rho_{\Sigma}$ satisfies
$\phi_{int}$. \qed


\end{enumerate}



\newcommand{\mk}{k^*}



By the above result, it suffices to consider only safety properties in
order to perform orchestration synthesis. However, it is a sufficient condition - given a fixed $k$, even if Lemma~3 fails for all possible assignment $\vec{v}$, one can not conclude that there exists no solution for the orchestration synthesis problem. One either reports \texttt{unknown} or repeats the search of feasible $\vec{v}$ by
enlarging $k$ and reapplying Lemma~3. 

We show next that, under some soft conditions, it is pointless to go beyond a reasonable bound. More precisely, if the domains of the parameters in input system $\mathcal{S}$ are bounded, then one can effectively compute a limit $\mk$ on $k$ such that if Lemma 3 is not applicable for $\mk$, then it will not be applicable on any other greater $k$. In practice, one only takes relatively small $k$ in orchestration synthesis, for instance~k=10.   

%such a limit is usually quite small (for instance 10).


%In theory, it suffices to check $k$ up to a certain threshold (see the result below for cases with bounded integer parameters), but in practice, even under small bounds (e.g., $k=10$) and without being able to find assignments for unknown parameters, the output might provide hints that the system should be restructured and such that hierarchical analysis can be applied.

%\obs{this para (from  ``When k is not large'' isn't clear to me: what does it mean ``k''  is not large enough? how does one decide that? So far, the reader  only has Lemma 3, which starts from an existing assigment. It  doesn't say anything about when such an assigment doesn't  exist. Strictly speaking, there's no \texttt{unknown} in Lemma 3. I  propose the following:} \new{We note that Lemma 3 gives a sufficient  condition. If for fixed $\vec{v}$, $k$ there exists a run reaching  either \sig{risk} or satisfying $dead$ then the lemma does not  apply. Still, one can synthesize a different $\vec{v}$ (obs: o far,  the reader has no clue about how to get $\vec{v}$, so maybe not put  explicitly ``syntetize a diff...''.)  or try a larger $k$. We show  next that, under some soft conditions, it is pointless to go beyond  a reasonable bound. More precisely, if the domains of the parameters  in input system $\mathcal{S}$ are bounded, then one can effectively  compute a limit $\mk$ on $k$ such that if Lemma 3 is not applicable  for $\mk$, then it will not be applicable on any other greater $k$. In practice, such a limit is usually quite small (for instance 10).}

%\obs{not clear what is meant by finding a controller.}

%\obs{replaced $\Delta$ by $\delta$ because $\Delta$ is already used for mapping interactions. btw, it's not quite clear to me why $\Delta$ is needed; we should be fine with defining interactions as  sets of ports...}

\begin{lemma} [$k$ with parameters of bounded integer domain, for interaction-level LTL properties]
%Given a system $\syst$ and an interaction-level property $\phi_{int}$,
Let all parameters in $\syst$ have bounded integer domains with common
upper bound $\lambda$ and $\delta$ be the number of regions in $\syst$
when all parameters within the location and guard conditions are assigned
$\lambda$. Let $|\mathcal{A}_{\neg\phi_{int}}|$ be the number of
locations in $\mathcal{A}_{\neg\phi_{int}}$, and $\eta$ be the number of discrete location combinations in $\mathcal{S}$, i.e.,  $\eta = |Q_1||Q_2|\dots|Q_m|$. Finally, let
 $\mk =
\delta^2\eta^2|\mathcal{A}_{\neg\phi_{int}}||\Sigma|+1$.  

Given $\vec{v}$ an
assignment of $V$, if there exists a time run of
$\mathcal{S}_{inv,\mk}(\vec{v})$ which reaches either \sig{risk} in
$C_{\neg\phi_{int},\mk}$ or a state where $\phi_{deadlock}(\vec{v})$
holds, then $\mathcal{S}(\vec{v})$ does not satisfy $\phi_{int}$.

%%   Given $\vec{v}$ an assignment of $V$,
%% $\mathcal{S}(\vec{v})$ does not satisfy $\phi_{int}$, if the following
%% conditions hold:
%% 	\begin{description}
%% 		\item[(i)] There exists a time run of $\mathcal{S}_{inv,k}(\vec{v})$ which reaches either the location \sig{risk} in $C_{\neg\phi_{int},k}$ or a state where $\phi_{deadlock}(\vec{v})$ holds. 
		
%% 		\item[(ii)] In condition (i), $k$ is of value $\mk = \delta^2|\mathcal{A}_{\neg\phi_{int}}||\Sigma|+1$.
%% 	\end{description}

%% \obs{why not collapse (i) and (ii) by substituting $k$ in (i) by
%%   $\mk$? Like this: Given $\vec{v}$ an assignment of $V$, if there
%%   exists a time run of $\mathcal{S}_{inv,\mk}(\vec{v})$ which reaches
%%   either the location \sig{risk} in $C_{\neg\phi_{int},\mk}$ or a
%%   state where $\phi_{deadlock}(\vec{v})$ holds, then
%%   $\mathcal{S}(\vec{v})$ does not satisfy $\phi_{int}$.}

	
%	 Given an assignment $\vec{v}$ of $V$,  if  Lemma~3 fails to hold when $k$ equals $\mk = \delta^2 |\mathcal{A}_{\neg\phi_{int}}||\Sigma|+1$, then $\vec{v}$ fails on Lemma~3, for all $k$ greater than $\mk$.
\end{lemma}

\proof (Sketch) Let $\rho$ be a time run of
$\mathcal{S}_{inv,\mk}(\vec{v})$ which reaches either \sig{risk} in
$C_{\neg\phi_{int},\mk}$ or a state where $\phi_{deadlock}(\vec{v})$
holds. We have two cases:
\begin{itemize}
\item \textbf{Case 1}: \sig{risk} is not reached, equally, $\rho$ reaches a state where $\phi_{deadlock}(\vec{v})$ holds. The deadlock of $\mathcal{S}_{inv,\mk}(\vec{v})$ under $\rho$ is irrelevant to the monitor component, as the monitor component does not hinder any execution apart from \sig{risk}.  Therefore, $\mathcal{S}(\vec{v})$ contains deadlock states, and 
 $\mathcal{S}(\vec{v})$ does not satisfy $\phi_{int}$, as reaching a deadlock state means that one can not create an  $\omega$-word from that time run. 
	
%\obs{i don't understand the footnote: what does it mean that all $\sigma \in \Sigma$ are considered? My intuition is that $\rho$ corresponds to a time run in $S(v)$ (i guess that, more generally, $S$ simulates $\mon{v}$ (any time run in $\mon{v}$ not ending in risk corresponds to a time run in $S(v)$), so we have a run in $S(v)$ which is deadlocked}.
	
	%%% CH: We need better explaination in Step 2 to say that the monitor really disables deadlock, apart from state \sig{risk}.
	
	%So applying $(\mk+1)$-th unroll does not help mediate the problem.
	
	\item \textbf{Case 2}: When \sig{risk} is reached in the $\mk$-th unroll, our
          proof objective is to demonstrate that with a prefix of a
          violating time run $\rho$ in $\mathcal{S}_{inv,\mk}(\vec{v})$ that visited one final state $s$ in
          $\mathcal{A}_{\neg\phi_{int}}$ for $\mk$ times, 
          one proves the existence of a time run $\rho'$ in $\mathcal{S}(\vec{v})$, by tailoring a fragment of $\rho$, such that the $\omega$-word of $\rho'$, when applying to $\mathcal{A}_{\neg\phi_{int}}$, guarantees to visit $s$ arbitrary times. 
          This is done with the help of two results: (1) the number of regions in a timed automaton is finite, and (2) pigeonhole principle.
	\begin{itemize}
	%	\item If Lemma 3 fails under $k=\mk$, then for all assignment $\vec{v}$  of $V$,  there exists one (violating) timed run $\rho_{vio}$ in $\mathcal{S}_{inv,k}(\vec{v})$,  whose time-prefix guarantees to visit at least a final state in $\mathcal{A}_{\neg\phi_{int}}$ for $\mk$ times. So it suffices to only consider one assignment of unknown variables. 
		%\obs{so far, the reader only knows how to compute a monitor, not also how to find controllers, no?}
		
		%\item From Step 3 of our construction, one can know that $\#$ actually represents elements in $\Sigma \setminus \Sigma_{\phi_{int}}$, i.e., $\#$ capture interactions not related to the property. This means that one can alternatively do the post-processing in Step 1 by replacing $\#$ by $|\Sigma \setminus \Sigma_{\phi_{int}}|$ edges, where each edge is labeled with $\sigma' \in \Sigma \setminus \Sigma_{\phi_{int}}$. Therefore, for every state of $\mathcal{A}_{\neg\phi_{int}}$, it can have at most $|\Sigma|$ distinct outgoing edges to the same destination. 
		
		\item When unknown variables are assigned with concrete values, the system is a timed automaton and the number of regions is finite. 
		The total number of regions is bounded by $\delta$. Recall the execution in monitor $C_{\neg \phi_{int},k}$ is actually reflecting the execution in the B\"uchi automaton $\mathcal{A}_{\neg\phi_{int}}$. Consider a discrete jump in the system. With a specific destination state $s$ in $\mathcal{A}_{\neg\phi_{int}}$, one can actually capture a discrete jump in $\mathcal{S}_{inv,k}(\vec{v})$ by only viewing its change in regions and  locations. To reflect such changes, we use
		 tuples $\langle(r_{source}, l_{source}, s_{source}),\sigma,(r_{dest}, l_{dest}, s)\rangle$, where $r_{source}$ and $r_{dest}$ are source and destination regions in $\mathcal{S}(\vec{v})$, $l_{source}$ and $l_{dest}$ are source and destination location in $\mathcal{S}(\vec{v})$, $s_{source}$ is the source state in $\mathcal{A}_{\neg\phi_{int}}$ with interaction $\sigma \in \Sigma$.
		The total number for all such $\langle(r_{source}, l_{source}, s_{source}),\sigma,(r_{dest}, l_{dest}, s)\rangle$ tuples is bounded by $\delta^2 \eta^2 |\mathcal{A}_{\neg\phi_{int}}| |\Sigma|$. 
		Therefore, when the violating time run $\rho$ visits a particular final state $s$ in $\mathcal{A}_{\neg\phi_{int}}$ for $\mk$ times, in the corresponding region representation, one particular tuple  $\langle(r_{source}, l_{source}, s_{source}),\sigma,(r_{dest}, l_{dest}, s)\rangle$ should have appeared twice (due to pigeonhole principle). The clock valuations associated to $l_{source}$, resp. $l_{dest}$ may be different in the two tuples. However, the corresponding states are region-equivalent and consequently bisimilar. Thanks to this, $\mathcal{S}$ can evolve region-bisimilarly  until the tuple $\langle(r_{source}, l_{source}, s_{source}),\sigma,(r_{dest}, l_{dest}, s)\rangle$ appears for the third time, and so on. While repeating this pattern a time run which visits $s$ infinitely often is constructed.  
%, although in the configuration, actual concrete clock readings can be different. 		
		%% \item Although the second state is different from the first due to the different clock readings, they are in the same location and region, meaning that two states are bisimilar. This implies that from the second  state, the system can evolve region-bisimilarly like the first concrete state, until the repeating tuple $\langle(r_{source}, l_{source}, s_{source}),\sigma,(r_{dest}, l_{dest}, s)\rangle$ appears for the third time. Again the third concrete state can be different from the first and the second, but it is bisimilar. Thus one can repeat the pattern and constructively generate a time run that visits $s$ infinitely often.  
		
		%Therefore, one can pump the sequence in between to create another time run $\rho'$, which guarantees to visit $s$ arbitrary many times. 
		
		%At each region, the monitor can actually be in any of the state. So one has (region, state-in-B\"uchi) pairs of size $\delta|\mathcal{A}_{\neg\phi_{int}}|$. 
		
		
		
	
		
		
		% for every possible assignment of unknown variables, the violation run should have at least visited one (region, state-in-B\"uchi) twice, and from there, use the same transition to go to another  (region, state-in-monitor) by the same interaction. 
		
		%\item Notice that our goal is further refined, as we want the twice visited be (region, final-state-in-B\"uchi). As this path visits one final state at least $\delta |\mathcal{A}_{\neg\phi_{int}}||\Sigma| +1$, at least for that final state, 
		
		
		%If between two identical occurrences, the final state which is touched $k$ times is also visited, then one can pump that segment to ensure that the final state is visited infinitely often.
		
	
		
	\end{itemize}
	
	
\end{itemize}



%nder $k=\mk$, for assignment $\vec{v}$ of $V$  either (1) the system $\mathcal{S}_{inv,\mk}(\vec{v})$ is deadlocked somewhere but \sig{risk} state in the $C_{\neg\phi_{int},k}$ is never touched \new{($\dead$ is satisfied)}, or (2) there exists one (violating) timed run $\rho_{vio}$ in $\mathcal{S}_{inv,\mk}(\vec{v})$, whose time-prefix guarantees to touch \sig{risk} in $C_{\neg\phi_{int},\mk}$, i.e., it visits at least a final state $s$ in $\mathcal{A}_{\neg\phi_{int}}$ for $\mk$ times. Therefore, we need to distinguish such two cases.
%whether \sig{risk} is touched in $C_{\neg\phi_{int},\mk}$. 






